Set Based Stochastic Subsampling

Deep models are designed to operate on huge volumes of high dimensional data such as images. In order to reduce the volume of data these models must process, we propose a set-based two-stage end-to-end neural subsampling model that is jointly optimized with an \textit{arbitrary} downstream task network (e.g. classifier). In the first stage, we efficiently subsample \textit{candidate elements} using conditionally independent Bernoulli random variables by capturing coarse grained global information using set encoding functions, followed by conditionally dependent autoregressive subsampling of the candidate elements using Categorical random variables by modeling pair-wise interactions using set attention networks in the second stage. We apply our method to feature and instance selection and show that it outperforms the relevant baselines under low subsampling rates on a variety of tasks including image classification, image reconstruction, function reconstruction and few-shot classification. Additionally, for nonparametric models such as Neural Processes that require to leverage the whole training data at inference time, we show that our method enhances the scalability of these models.

==> algorithms/fixed_size_sss_bkup.tex <==
\begin{algorithm*}[tb]
   \caption{\small Fixed Size Subset Selection}
   \label{fixed-size-selection}
   \begin{tabularx}{\textwidth}{ll}
    \textbf{Input} & $k$(subset size), $q$(\# elements selected at each iteration),
	  $D=\{d_1,d_2,\ldots,d_n\}$ (Full Set)\\
    \textbf{Output} & $D_s=\{s_1, s_2,\ldots, s_k\}$ (selected subset)
   \end{tabularx}

  \begin{algorithmic}[1]
    \FUNCTION{STOCHASTIC SUBSET SELECTION$(k,q,D)$}
      \STATE $(\pi_1, \pi_2, \ldots, \pi_n) \leftarrow (\rho(d_i, r(D)), \ldots, \rho(d_n, r(D)))$
      \STATE $z_i \sim \text{Ber}(\pi_i) \text{ for } i=1, \ldots, n.$
      \STATE $D_c \leftarrow \{d_i \text{ for } i=1:n \text{ if } z_1\}$	
      \STATE $D_s  \leftarrow \emptyset$
      \FOR{$i=1$ {\bfseries to} $k/q$}
	\STATE $D_s \leftarrow D_s \cup \text{AUTOSELECT}(q,D_s, D_c)$
      \ENDFOR
    \ENDFUNCTION

    \FUNCTION{AUTOSELECT$(q, D\_s, D\_c)$}
      \STATE $C = \{w_1, w_2, \ldots, w_m\} \leftarrow D_c \setminus D_s$
      \STATE $(p_1, p_2, \ldots, p_m) \leftarrow (f(w_1, D_c, D_s), f(w_2, D_c, D_s), \ldots f(w_m, D_c, D_s))$
      \STATE $(p_1, p_2, \ldots, p_m) \leftarrow (p_1, p_2, \ldots, p_m) / \sum_{j=1}^{m} p_j$
      \STATE $Q \leftarrow \text{Select } q \text{ elements from } C \text{ with probability } (p_1, p_2, \ldots, p_m)$
      \STATE $\text{return } Q$
    \ENDFUNCTION
  \end{algorithmic}
\end{algorithm*}


==> figures/instance_selection.tex <==
\begin{figure*}
    \centering
		\includegraphics[width=\linewidth]{images/reconstruction_samples/distill_samples_row.pdf}
		\vspace{-0.2in}
		\caption{\small Representative Samples from a dataset of size 200 by subset selection models. }
		\vspace{-0.1in}
		\label{fig:instance_selection}
\end{figure*}	


==> figures/miniimagenet.tex <==
\begin{wrapfigure}{r}{0.25\textwidth}
    \centering
    \vspace{-0.2in}
    \includegraphics[width=0.25\textwidth]{images/function/plots/miniimagenet.pdf}
    \vspace{-0.1in}
    \caption{\small Accuracy on \textit{mini}Imagenet.}
    \label{fig:miniimagenet}
\end{wrapfigure}

==> figures/model_overview.tex <==
\begin{figure*}
    \centering
    \includegraphics[width=1.0\textwidth]{images/concept_images/method_sss.pdf}
    \vspace{-0.25in}
    \caption[Model Overview]{\small \textbf{Overview.} Two-stages of subsampling. \textbf{(a)} Construction of candidate subset $D_c$ with sampling mask for each instance from Bernoulli distribution. \textbf{(b)} Iteratively sampling elements from the candidate set with multinomial distribution to construct the subset $D_s$.} 
    \vspace{-0.2in}
    \label{overview}
\end{figure*}



==> figures/reconstruction_samples.tex <==
% \begin{figure*}
% \vspace{-0.1in}
% 	\begin{subfigure}{1.0\textwidth}
% 		\centering
% 		\includegraphics[width=\linewidth]{images/reconstruction_samples/reconstruction_sample.png}
% 		\caption{\small CelebA reconstruction samples with varying the number of pixels.}
% 		\label{reconstruction-celeba}
% 	\end{subfigure}
% 	\begin{subfigure}{1.0\textwidth}
% 		\centering
% 		\includegraphics[width=\linewidth]{images/reconstruction_samples/distill_samples_row.pdf}
% 		\caption{\small Instance Selection Samples from a dataset of size 200. Here, SSS selects samples that are most representative of the input dataset resulting in better FID score. An example with the full 200 elements together with samples selected in both the Canditate Selection and 
% 		Autoregressive Selection Stages is provided in the Supplementary File.}
% 		\label{row_figs}
% 	\end{subfigure}
% \end{figure*}


\begin{figure*}[t]
    \centering
    \includegraphics[width=\linewidth]{images/reconstruction_samples/reconstruction_sample.png}
    \vspace{-0.25in}
	\caption{\small CelebA reconstruction samples with varying the number of pixels.}
	\label{reconstruction-celeba}
\end{figure*}

==> rebuttal/table.tex <==
\begin{wrapfigure}{t}{0.2\textwidth}
\small
\centering
\vspace{-0.15in}
\captionof{table}{\small Acc. with \textbf{200} out of 1024 pixels on OCT.}
\resizebox{0.2\textwidth}{!}{
\renewcommand{\arraystretch}{0.75}
\renewcommand{\tabcolsep}{0.5mm}
\begin{tabular}{cccc|c}
\toprule
Random & INVASE & DPS & \textbf{SSS} & Full \\ 
\midrule
38.80 & 41.80 & 76.70 & \textbf{85.90} & 95.50\\
\bottomrule
\end{tabular}
}
\vspace{-0.17in}
\label{tab-exp}
\end{wrapfigure}


==> sections/broader_impact.tex <==
\section{Broader Impact}
Given that modern machine learning and deep learning algorithms are increasingly being deployed on mobile, embedded and edge devices, the capability to process data in real-time on such resource constrained devices will become a necessity. Our work, which seeks to reduce the volume of such data, utilizes a two stage stochastic subset selection module that learns to select relevant subsets of input data or the selection of a subset of a given dataset. This has practical applications on conventional hardware given that we can significantly reduce both the memory and computational footprints of many deep learning models in tasks such as object classification and reconstruction. 
